DeepFloat: Resource-Efficient Dynamic Management of Vehicular Floating Content

Opportunistic communications are expected to playa crucial role in enabling context-aware vehicular services. A widely investigated opportunistic communication paradigm for storing a piece of content probabilistically in a geographica larea is Floating Content (FC). A key issue in the practical deployment of FC is how to tune content replication and caching in a way which achieves a target performance (in terms of the mean fraction of users possessing the content in a given region of space) while minimizing the use of bandwidth and host memory. Fully distributed, distance-based approaches prove highly inefficient, and may not meet the performance target,while centralized, model-based approaches do not perform well in realistic, inhomogeneous settings. In this work, we present a data-driven centralized approach to resource-efficient, QoS-aware dynamic management of FC.We propose a Deep Learning strategy, which employs a Convolutional Neural Network (CNN) to capture the relationships between patterns of users mobility, of content diffusion and replication, and FC performance in terms of resource utilization and of content availability within a given area. Numerical evaluations show the effectiveness of our approach in deriving strategies which efficiently modulate the FC operation in space and effectively adapt to mobility pattern changes over time.

==> 02_related_work.tex <==
\section{Related Work}
\label{rel_wor}
Machine learning approaches for vehicular networks application have increased due to their appealing characteristics to deal with massive datasets and modeling realistic scenarios of high uncertainty and extract meaningfully content from them. In~\cite{TaP2016} authors showed how a \textit{k}-means algorithm could guide the design of a control strategy for data congestion by clustering the multidimensional feature space of VANETs.~\cite{YLL2018} gives an overall view of the recent application of machine learning in vehicular networks including novel deep learning approaches to the prediction of traffic flow and local data storage.



A performance modeling of the Floating Content paradigm for vehicular networks is presented in~\cite{itc_journal}. In the cited work, authors applied a variation of the Random Waypoint Model to estimate the success ratio based on the Anchor Zone radius (i.e., the probability for a node to receive the content during its sojourn within a circular communication area). 
In~\cite{ours2017mobiworld}, authors proposed two algorithms, which use both centralized and distributed approach for data collection, to set the radius of a circular Anchor Zone while achieving targets of performance. A first cognitive approach for FC dimensioning was proposed in~\cite{wain_2018}. In the cited paper, authors provided a content sharing system to optimize replication and caching strategies within the communication area defined by a convolutional neural network. Numerical evaluations in~\cite{wain_2018} take into account only synthetic mobility such as Manhattan mobility. Moreover, the optimization is made without accounting for infrastructure support cost.

Our work extends~\cite{wain_2018} providing a new formulation of the problem, optimizing seeding strategy, simulating in real vehicular patterns, and model evolution. The new formulation considers both mobile user and infrastructure resources. Despite~\cite{wain_2018}, the system provides the optimal seeding strategy for the given mobility pattern. In this new version, the system is shaped to provide a temporal strategy evaluated over real data from~\cite{lux} and compared with the state-of-the-art FC model.


%Authors in~\cite{floating} have introduced Floating Content (FC) revealing the minimum conditions to keep the content viable within the Anchor Zone (AZ). A first step to optimize the AZ, in term of resources employed, has been presented in~\cite{ours2017mobiworld}. In the cited work, authors have optimized a circular AZ, analytically modeled. 
%Sebastian wrote this aiming to answer: Why machine learning, particularly deep learning and specifically for this work a CNN, feel free to modify/extend it/delete it%



==> leftovers_march.tex <==
Deep learning algorithm models maps as input to a class label using a back-propagation algorithm to adjust the weights of the network~\cite{goodfellow2016deep}. Convolutional neural networks (CNNs) are a subset of deep learning algorithms that learn spatial correlations between grid-like input data. The first layers in this CNN architectures learn basic visual primitives such as lines and edges, and then builds more complex filters using non-linear combination of the first layer filters. 

CNNs have shown disruptive performance not only in computer vision but also in speech recognition and natural language processing tasks~\cite{LBY2015}. 



infrastructure collects UE mobility data according to a fixed sampling period. 
%We assume UEs communicate their position to the infrastructure over time.

As we explained, we assume that the application floating period is partitioned into intervals

%The information stored in the elements of $\mathbf{P}$ are listed in Table~\ref{Tab1:features}. 
%Note that we have chosen as link features those parameters which are typically chosen to parameterize, in practical settings, the existing analytical models of FC performance \cite{ours2017mobiworld,itc29}.\\
% a \textit{randomization} is applied to derive the communication features $\mathbf{P_c}$. The randomization technique consists to apply random strategies of $\mathbf{A}$, and random seeding where $a$ and $b$ are greater than zero. The collected features are the number of nodes with content $n^c$, and the number of nodes transmitting $\gamma$, in each link. These features are required for the following reasons: application target achievement, cost function evaluation, and features/label correlation.
% \subsubsection{Data transformation (inutile)}
% After label generation, the \textit{data transformation} step consists in deriving, for all of the above parameters, an average value for each link and in every time interval into which \textbf{the mysterious floating period} has been divided.
%denote the set of all those pairs produced in the offline setup phase.  
% The next step is to manipulate these data (block \textit{data transformation}) to prepare it for the learning process. In this stage, data are averaged over the interval time defined by the application and normalized by feature. This block contains the feature set of all links (called \textit{links feature vector}, denoted as $\mathbf{P}$, and listed in Table~\ref{Tab1:features}), and the related strategy $\mathbf{A}$. The link features vector
%The above steps are made offline, i.e. they are not based on the application. 
% denoted as $\mathbf{P_m}$, in the given set of road links (block \textit{database}).  %via OpenStreetMap~\cite{OpenStreetMap}. 
%  The mobility features $\mathbf{P_m}$ are (come le hai scelte?) 

%In the deployment phase, to ensure an optimal strategy $\mathbf{A^n}$ for the predicted mobility, we assume the minimum floating lifetime to be greater or equal than the minimum interval length $d_t$.
%{\bf MAM: perche` apice e pedice a P? L'apice di A non dovrebbe essere *, come nella pagina precedente?}

% \subsection{Training process and validation }

% In what follows, we describe our CNN algorithm. It consists in a supervised multi-labelled learning process, in which a CNN is used to relate the mobility features $\mathbf{P_m}$ to their labels $\mathbf{P_c}$ and $\mathbf{A}$.

% For such learning process, the training set consists of the set $\Pi$. The size of the set is chosen as a compromise between computational load (and hence time to complete the CNN training) and accuracy of the output.


% Following the training period where the CNN learned the connection $(\mathbf{P},\mathbf{A})$, the CNN goes to a validation process. 

% The procedure is the following. 
% \begin{itemize}
% \item The mobility features vector $\mathbf{P_{m}}$ is given as input to the CNN.
% {\bf MAM: anche qui (e sotto), perche` apice e pedice? tra l'altro, ho messo in bf, come sempre - era in corsivo}
% \item The CNN distinguishes those inputs that lead to a strategy $\mathbf{A}$ that satisfies the constraint on success ratio \eref{eq:availability_zoi}. Specifically, the CNN checks if the input $\mathbf{P_{m}^{new}}$ is in the learning dataset. In case of success, the CNN provides the respective output, which respects the application target, with the minimum resource usage. CNN outputs can be the vector of links set to zero, which means that for the given mobility no configuration $\mathbf{A}$ can be applied. Note that, the input all-on strategy $\mathbf{A}=(1,1)$, for each link in each interval, is in the training set.

% \item In case the input is not in the training set, the CNN provides all outputs related to the given mobility. These configurations will be studied via simulation to check which one meets the application targets. Then, $(\mathbf{P},min(\mathbf{A}))$ is added to the machine learning set. Where $min(\mathbf{A})$ is the most efficient configuration (i.e., the configuration with the minimum cost of Problem~\ref{prob:1}).  
% \end{itemize} 

% It is important to highlight that in this stage we do not aim to reach the maximum accuracy (to avoid over-fitting issues). As a matter of fact, the perfect machine tuning requires that the validation and the test accuracy are the same~\cite{goodfellow2016deep}.

%The supervised learning process uses a CNN to relate the link features $\mathbf{P}$ to their labels $\mathbf{A}$. Rather $\mathbf{P_m},\mathbf{P_c},$\mathbf{A}$.

%The training set consists of $N$ couples of matrices $(\mathbf{P},\mathbf{A})$, where the size $N$ is chosen as a compromise between computational load (and hence time to complete the CNN training) and accuracy of the output.
%That is, the mean node speed, the mean number of nodes in a link, the mean rate of contacts in a link, and the mean duration of each contact. In addition to these parameters, relative to mobility, we have also considered those parameters which allow computing the cost function (\ref{eq:objectivefunction}), i.e. the mean number of nodes with content in a link, and and the mean number of concurrent content exchanges in a link.  
%Our choice as link features has been In what follows, we ahve chosen Examples of mobility features are the total number of cars or the average vehicles speed in each the road links. Note that these features can be predicted from past mobility data. 
%The set of features related to the communication part of the system may include such parameters as the number of nodes with content, or the number of nodes in contact (i.e., within transmission range of each other). 
%\textbf{Communication features can be obtained via simulation. or by direct measurement, analogously to the mobility features}  
% Table~\ref{Tab1:features} shows a possible choice for such parameters, but our approach can be extended to other choices of parameters.
% \begin{table}[t!]
% \small
% \caption{Link Features nector $P_{l,t}$}
% \centering
% \begin{tabular}{ |c|c|c|}
%  \hline
%  Name&   Unit& Description \\
%  \hline
%  \hline
%  $n^c_{l,t}$ &  & \# nodes with content\\
%  \hline
%  $n^{nc}_{l,t}$ &  & \# nodes without content\\
%  \hline
%  $\lambda_{l,t}$ &  & \# nodes in contact\\
%   \hline
%  $\tau_{l,t}$ & $[s]$ &  contact time\\
%  \hline
%  $v_{l,t}$ &  $[m/s]$& nodes average speed\\
%  \hline
%   $\gamma_{l,t}$ &  & \# nodes transmitting\\
%  \hline
% % $r$ &  meters& vehicle transmission radius\\ 
% % \hline
% \end{tabular}
% \label{Tab1:features}
% \end{table}
%The learning process uses a CNN to relate the link features $\mathbf{P}$ to their labels $\mathbf{A}$. 
%The process is trai the CNN to distinguish those inputs that lead to a strategy $\mathbf{A}$ that satisfies the constraint on success ratio \eref{eq:availability_zoi}), is as follows.
% We assume such a dataset is built by simulations based on historical mobility data, and increased progressively during the operations. In order to train the CNN to distinguish those inputs which lead to a feasible strategy $\mathbf{A}$ (i.e. to a strategy which satisfies the constraint on success ratio \eref{eq:availability_zoi}), to each couple $(\mathbf{P},\mathbf{A})$ in the dataset it is associated (by simulations or direct measurements) a binary variable, indicating whether \eref{eq:availability_zoi} is satisfied.
% puts satisfy the desired message availability . To accomplish this task, a data preprocessing is applied. In particular, the feature vector $p^{com}$ reveals if the required application performance has been achieved. In case of failure, i.e., if the application performance constraint is not satisfied, the machine learns that the configuration $A$ for that specific input is not feasible. Otherwise, if the requirement is fulfilled, the machine learns the relation between the given $A$ and $P$ or rather the triple $(p^{mob},p^{com},A)$. 

% %An example of output shape and parameter number, used in the Section~\ref{N-e}, is listed in Table~\ref{tab:cnn_arc}.
% %
% %
% \begin{table}[t]
% %\footnotesize
% \begin{center}
% \caption{Structure of the Convolutional Neural Network on $162$ road links.}
% \begin{tabular}{ c c c}
 
%   Layer & Shape & Param \#\\
%   \hline
%   \hline
%     $Conv2D$ & $(160,2,16)$ &160\\
%   \hline
%     $Activation$&$(160,2,16)$ &0\\
%   \hline
%     $MaxPooling2D$&(80,1,16)&0\\
%   \hline
%     $Conv2D$ & $(80,2,16)$ &272\\
%   \hline
%     $Activation$&$(80,1,16)$ &0\\
%   \hline
%     $Flatten$ &(1280)&0\\
%   \hline
%     $Dense$&(64)&81984\\
% \hline
%     $Activation$&$(64)$ &0\\
%   \hline
%     $Dropout$&$(64)$ &0\\
%   \hline
%     $Dense$&$(162)$&10530\\
% \hline
%     $Activation$&$(162)$ &0
%   \label{tab:cnn_arc}
% \end{tabular}
% \end{center}
% \normalsize
% \vspace{-0.2in}
% \end{table}




\textbf{Implementation details about the training phase} The CNN does not process its inputs one-at-a-time. In order to increase throughput, the CNN process the data in \textit{batches}. A batch is a $N_l$ by $N_f$ matrix, with $N_l$ and $N_f$ the numbers of road links and features, respectively. Since no spatial relation is passed as input data, batches are shuffled. The number of iterations, i.e. the number of time that a batch must pass through the CNN (forward and backward) \textbf{to accomplish an epoch} \gr{?}, is chosen according to the batch size \gr{how?}. The goal of this procedure is to fine tune the internal CNN parameters, by learning several configurations and the respective spatial information. \gr{?}


It is important to note that generally an analytical model applied to a real scenario has lower precision with respect to the application to a synthetic environment with features that match the model. By using a ML approach, the quality of the performance depends only on the quality of data and the technique used to process them.


In such a scenario, our approach is compared to other ML techniques, and to an analytical approach that considers a circular area around the ZOI (i.e., it considers the ZOI at the center of a circular area over which we set probability $1$ for both replication and caching). 

